Systematic study of amorphous 2D graphene, silicene and silicon carbide: Investigation of structural, electronic, optical and vibrational properties

Although 2D solids and their vdW heterostructures have garnered much attention recently, their amorphous forms have been less explored. We present a detailed analysis of the structural, electronic, and thermal properties of 2D amorphous graphene (A-Gra), silicene (A-Si), and silicon carbide (A-SiC) using Classical Molecular Dynamics (MD) simulations and first-principles calculations. Our results showed that A-Gra is planar at 0 K and wrinkled at 300 K, like its crystalline counterpart. At both temperatures, it can form stable vdW solids while maintaining metallic behavior. We also demonstrate that A-Si creates covalent bonds in layered structures while keeping its metallicity. Its optical spectrum is blue-shifted in parallel polarization relative to crystalline silicene, and its plasmon peak is in the UV range with six-times higher intensity. Furthermore, we show that 2D silicon carbide can be stabilized as a single layer or in layered structures with bonding between Si atoms only. A-SiC's plasmon peak is in the UV range. All three structures' optical spectra are observed as red-shifted compared to their crystalline counterparts, and their absorption spectra range from IR to UV. Their common heat carriers are extendons, especially diffusions, and their thermal conductivity is calculated to be lower than that of their crystalline counterparts. Our findings suggest that the uneven charge distributions around local ring structures in all three systems can be exploited in future electronic, thermo-electric, and opto-electronic devices with local functionality.

==> preamble.tex <==
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage[left=23mm,right=13mm,top=35mm,columnsep=15pt]{geometry} 
\usepackage{adjustbox}
\usepackage{placeins}
\usepackage[T1]{fontenc}
\usepackage{lipsum}
\usepackage{csquotes}
